muSR and Magnetometry Study of the Type-I Superconductor BeAu

We present muon spin rotation and relaxation (muSR) measurements as well as demagnetising field corrected magnetisation measurements on polycrystalline samples of the noncentrosymmetric superconductor BeAu. From muSR measurements in a transverse field, we determine that BeAu is a type-I superconductor with Hc = 256 Oe, amending the previous understanding of the compound as a type-II superconductor. To account for demagnetising effects in magnetisation measurements, we produce an ellipsoidal sample, for which a demagnetisation factor can be calculated. After correcting for demagnetising effects, our magnetisation results are in agreement with our muSR measurements. Using both types of measurements we construct a phase diagram from T = 30 mK to Tc = 3.25 K. We then study the effect of hydrostatic pressure and find that 450 MPa decreases Tc by 34 mK, comparable to the change seen in type-I elemental superconductors Sn, In and Ta, suggesting BeAu is far from a quantum critical point accessible by the application of pressure.

==> BeAu_Manuscript_v1_bib.tex <==
@article{Hayashi2006,
  title = {Temperature dependence of the superfluid density in a noncentrosymmetric superconductor},
  author = {Hayashi, N. and Wakabayashi, K. and Frigeri, P. A. and Sigrist, M.},
  journal = {Phys. Rev. B},
  volume = {73},
  issue = {2},
  pages = {024504},
  numpages = {9},
  year = {2006},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.73.024504},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.73.024504}
}

@article{Sigrist2007,
title = "Superconductivity in non-centrosymmetric materials",
journal = "Journal of Magnetism and Magnetic Materials",
volume = "310",
number = "2, Part 1",
pages = "536 - 540",
year = "2007",
note = "Proceedings of the 17th International Conference on Magnetism",
issn = "0304-8853",
doi = "https://doi.org/10.1016/j.jmmm.2006.10.141",
url = "http://www.sciencedirect.com/science/article/pii/S0304885306013175",
author = "Manfred Sigrist and D.F. Agterberg and P.A. Frigeri and N. Hayashi and R.P. Kaur and A. Koga and I. Milat and K. Wakabayashi and Y. Yanase",
keywords = "Unconventional superconductivity, Spin–orbit coupling, Non-centrosymmetric materials"

}


@article{Takimoto2009,
author = {Takimoto ,Tetsuya and Thalmeier ,Peter},
title = {Triplet Cooper Pair Formation by Anomalous Spin Fluctuations in Non-centrosymmetric Superconductors},
journal = {Journal of the Physical Society of Japan},
volume = {78},
number = {10},
pages = {103703},
year = {2009},
doi = {10.1143/JPSJ.78.103703},

URL = { 
        https://doi.org/10.1143/JPSJ.78.103703
    
}
}

@article{Bonalde2005,
  title = {Evidence for Line Nodes in the Superconducting Energy Gap of Noncentrosymmetric ${\mathrm{CePt}}_{3}\mathrm{Si}$ from Magnetic Penetration Depth Measurements},
  author = {Bonalde, Ismardo and Br\"amer-Escamilla, Werner and Bauer, Ernst},
  journal = {Phys. Rev. Lett.},
  volume = {94},
  issue = {20},
  pages = {207002},
  numpages = {4},
  year = {2005},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.94.207002},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.94.207002}
}

@article{Mukuda2008,
  title = {Enhancement of Superconducting Transition Temperature due to the Strong Antiferromagnetic Spin Fluctuations in the Noncentrosymmetric Heavy-Fermion Superconductor ${\mathrm{CeIrSi}}_{3}$: A $^{29}\mathrm{Si}$ NMR Study under Pressure},
  author = {Mukuda, H. and Fujii, T. and Ohara, T. and Harada, A. and Yashima, M. and Kitaoka, Y. and Okuda, Y. and Settai, R. and Onuki, Y.},
  journal = {Phys. Rev. Lett.},
  volume = {100},
  issue = {10},
  pages = {107003},
  numpages = {4},
  year = {2008},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.100.107003},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.100.107003}
}

@article{Bonalde2009,
  title = {Possible two-gap behavior in noncentrosymmetric superconductor ${\text{Mg}}_{10}{\text{Ir}}_{19}{\text{B}}_{16}$: A penetration depth study},
  author = {Bonalde, I. and Ribeiro, R. L. and Br\"amer-Escamilla, W. and Mu, G. and Wen, H. H.},
  journal = {Phys. Rev. B},
  volume = {79},
  issue = {5},
  pages = {052506},
  numpages = {4},
  year = {2009},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.79.052506},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.79.052506}
}

@article{Bauer2010,
  title = {Unconventional superconducting phase in the weakly correlated noncentrosymmetric ${\text{Mo}}_{3}{\text{Al}}_{2}\text{C}$ compound},
  author = {Bauer, E. and Rogl, G. and Chen, Xing-Qiu and Khan, R. T. and Michor, H. and Hilscher, G. and Royanian, E. and Kumagai, K. and Li, D. Z. and Li, Y. Y. and Podloucky, R. and Rogl, P.},
  journal = {Phys. Rev. B},
  volume = {82},
  issue = {6},
  pages = {064511},
  numpages = {5},
  year = {2010},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.82.064511},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.82.064511}
}

@article{Nishiyama2007,
  title = {Spin Triplet Superconducting State due to Broken Inversion Symmetry in ${\mathrm{Li}}_{2}{\mathrm{Pt}}_{3}\mathrm{B}$},
  author = {Nishiyama, M. and Inada, Y. and Zheng, Guo-qing},
  journal = {Phys. Rev. Lett.},
  volume = {98},
  issue = {4},
  pages = {047002},
  numpages = {4},
  year = {2007},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.98.047002},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.98.047002}
}

@article{Yuan2006,
  title = {$S$-Wave Spin-Triplet Order in Superconductors without Inversion Symmetry: ${\mathrm{Li}}_{2}{\mathrm{Pd}}_{3}\mathrm{B}$ and ${\mathrm{Li}}_{2}{\mathrm{Pt}}_{3}\mathrm{B}$},
  author = {Yuan, H. Q. and Agterberg, D. F. and Hayashi, N. and Badica, P. and Vandervelde, D. and Togano, K. and Sigrist, M. and Salamon, M. B.},
  journal = {Phys. Rev. Lett.},
  volume = {97},
  issue = {1},
  pages = {017006},
  numpages = {4},
  year = {2006},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.97.017006},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.97.017006}
}

@article{Isobe2016,
  title = {Superconductivity in noncentrosymmetric ${\mathrm{SrAuSi}}_{3}$},
  author = {Isobe, Masaaki and Arai, Masao and Shirakawa, Naoki},
  journal = {Phys. Rev. B},
  volume = {93},
  issue = {5},
  pages = {054519},
  numpages = {11},
  year = {2016},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.93.054519},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.93.054519}
}

@article{Anand2011,
  title = {Specific heat and $\ensuremath{\mu}$SR study on the noncentrosymmetric superconductor LaRhSi${}_{3}$},
  author = {Anand, V. K. and Hillier, A. D. and Adroja, D. T. and Strydom, A. M. and Michor, H. and McEwen, K. A. and Rainford, B. D.},
  journal = {Phys. Rev. B},
  volume = {83},
  issue = {6},
  pages = {064522},
  numpages = {9},
  year = {2011},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.83.064522},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.83.064522}
}

@article{Barker2015,
  title = {Unconventional Superconductivity in ${\mathrm{La}}_{7}{\mathrm{Ir}}_{3}$ Revealed by Muon Spin Relaxation: Introducing a New Family of Noncentrosymmetric Superconductor That Breaks Time-Reversal Symmetry},
  author = {Barker, J. A. T. and Singh, D. and Thamizhavel, A. and Hillier, A. D. and Lees, M. R. and Balakrishnan, G. and Paul, D. McK. and Singh, R. P.},
  journal = {Phys. Rev. Lett.},
  volume = {115},
  issue = {26},
  pages = {267001},
  numpages = {5},
  year = {2015},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.115.267001},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.115.267001}
}

@article{Hillier2009,
  title = {Evidence for Time-Reversal Symmetry Breaking in the Noncentrosymmetric Superconductor ${\mathrm{LaNiC}}_{2}$},
  author = {Hillier, A. D. and Quintanilla, J. and Cywinski, R.},
  journal = {Phys. Rev. Lett.},
  volume = {102},
  issue = {11},
  pages = {117007},
  numpages = {4},
  year = {2009},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.102.117007},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.102.117007}
}

@article{Iwamoto1998,
title = "Microscopic measurements in 139La-NQR of the ternary carbide superconductor LaNiC2",
journal = "Physics Letters A",
volume = "250",
number = "4",
pages = "439 - 442",
year = "1998",
issn = "0375-9601",
doi = "https://doi.org/10.1016/S0375-9601(98)00839-1",
url = "http://www.sciencedirect.com/science/article/pii/S0375960198008391",
author = "Y. Iwamoto and Y. Iwasaki and K. Ueda and T. Kohara",
keywords = "Ternary carbide superconductor, LaNiC, NQR, Nuclear spin relaxation rate"
}

@article{Sugawara2007,
  title = {Anomalous superconducting-gap symmetry of noncentrosymmetric ${\mathrm{La}}_{2}{\mathrm{C}}_{3}$ observed by ultrahigh-resolution photoemission spectroscopy},
  author = {Sugawara, K. and Sato, T. and Souma, S. and Takahashi, T. and Ochiai, A.},
  journal = {Phys. Rev. B},
  volume = {76},
  issue = {13},
  pages = {132512},
  numpages = {4},
  year = {2007},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.76.132512},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.76.132512}
}

@article{Samokhin2008,
  title = {Gap structure in noncentrosymmetric superconductors},
  author = {Samokhin, K. V. and Mineev, V. P.},
  journal = {Phys. Rev. B},
  volume = {77},
  issue = {10},
  pages = {104520},
  numpages = {9},
  year = {2008},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.77.104520},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.77.104520}
}

@article{Suter2012,
title = "Musrfit: A Free Platform-Independent Framework for μSR Data Analysis",
journal = "Physics Procedia",
volume = "30",
pages = "69 - 73",
year = "2012",
note = "12th International Conference on Muon Spin Rotation, Relaxation and Resonance (μSR2011)",
issn = "1875-3892",
doi = "https://doi.org/10.1016/j.phpro.2012.04.042",
url = "http://www.sciencedirect.com/science/article/pii/S187538921201228X",
author = "A. Suter and B.M. Wojek",
keywords = "μSR data analysis"
}

@article{Agterberg1999,
  title = {Conventional mechanisms for exotic superconductivity},
  author = {Agterberg, D. F. and Barzykin, Victor and Gor'kov, Lev P.},
  journal = {Phys. Rev. B},
  volume = {60},
  issue = {21},
  pages = {14868--14871},
  numpages = {0},
  year = {1999},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.60.14868},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.60.14868}
}

@article{Shimozawa2014,
  title = {Controllable Rashba Spin-Orbit Interaction in Artificially Engineered Superlattices Involving the Heavy-Fermion Superconductor ${\mathrm{CeCoIn}}_{5}$},
  author = {Shimozawa, M. and Goh, S. K. and Endo, R. and Kobayashi, R. and Watashige, T. and Mizukami, Y. and Ikeda, H. and Shishido, H. and Yanase, Y. and Terashima, T. and Shibauchi, T. and Matsuda, Y.},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  issue = {15},
  pages = {156404},
  numpages = {5},
  year = {2014},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.156404},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.156404}
}


@article{Luke1998,
	Author = {Luke, G. M. and Fudamoto, Y. and Kojima, K. M. and Larkin, M. I. and Merrin, J. and Nachumi, B. and Uemura, Y. J. and Maeno, Y. and Mao, Z. Q. and Mori, Y. and Nakamura, H. and Sigrist, M.},
	Date = {1998/08/06/online},
	Journal = {Nature},
	L3 = {10.1038/29038; },
	Month = {08},
	Pages = {558 EP  -},
	Publisher = {Macmillan Magazines Ltd. SN  -},
	Title = {Time-reversal symmetry-breaking superconductivity in Sr2RuO4},
	Ty = {JOUR},
	Url = {http://dx.doi.org/10.1038/29038},
	Volume = {394},
	Year = {1998},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/29038}}

@article{Xia2006,
  title = {High Resolution Polar Kerr Effect Measurements of ${\mathrm{Sr}}_{2}{\mathrm{RuO}}_{4}$: Evidence for Broken Time-Reversal Symmetry in the Superconducting State},
  author = {Xia, Jing and Maeno, Yoshiteru and Beyersdorf, Peter T. and Fejer, M. M. and Kapitulnik, Aharon},
  journal = {Phys. Rev. Lett.},
  volume = {97},
  issue = {16},
  pages = {167002},
  numpages = {4},
  year = {2006},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.97.167002},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.97.167002}
}


@article{Luke1993,
  title = {Muon spin relaxation in ${\mathrm{UPt}}_{3}$},
  author = {Luke, G. M. and Keren, A. and Le, L. P. and Wu, W. D. and Uemura, Y. J. and Bonn, D. A. and Taillefer, L. and Garrett, J. D.},
  journal = {Phys. Rev. Lett.},
  volume = {71},
  issue = {9},
  pages = {1466--1469},
  numpages = {0},
  year = {1993},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.71.1466},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.71.1466}
}

@article{Dereotier1995,
title = "Absence of zero field muon spin relaxation induced by superconductivity in the B phase of UPt3",
journal = "Physics Letters A",
volume = "205",
number = "2",
pages = "239 - 243",
year = "1995",
issn = "0375-9601",
doi = "https://doi.org/10.1016/0375-9601(95)00548-H",
url = "http://www.sciencedirect.com/science/article/pii/037596019500548H",
author = "P.Dalmas de Réotier and A. Huxley and A. Yaouanc and J. Flouquet and P. Bonville and P. Imbert and P. Pari and P.C.M. Gubbens and A.M. Mulders"
}

@article{Sigrist1998,
author = {Sigrist, Manfred},
title = {Time-Reversal Symmetry Breaking States in High-Temperature Superconductors},
journal = {Progress of Theoretical Physics},
volume = {99},
number = {6},
pages = {899-929},
year = {1998},
doi = {10.1143/PTP.99.899},
URL = {http://dx.doi.org/10.1143/PTP.99.899},
eprint = {/oup/backfile/content_public/journal/ptp/99/6/10.1143/ptp.99.899/2/99-6-899.pdf}
}

@article{Heffner1990,
  title = {New phase diagram for (U,Th)${\mathrm{Be}}_{13}$: A muon-spin-resonance and ${\mathrm{H}}_{\mathit{C}1}$ study},
  author = {Heffner, R. H. and Smith, J. L. and Willis, J. O. and Birrer, P. and Baines, C. and Gygax, F. N. and Hitti, B. and Lippelt, E. and Ott, H. R. and Schenck, A. and Knetsch, E. A. and Mydosh, J. A. and MacLaughlin, D. E.},
  journal = {Phys. Rev. Lett.},
  volume = {65},
  issue = {22},
  pages = {2816--2819},
  numpages = {0},
  year = {1990},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.65.2816},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.65.2816}
}

@article{Aoki2007,
author = {Aoki ,Yuji and Tayama ,Takashi and Sakakibara ,Toshiro and Kuwahara ,Keitaro and Iwasa ,Kazuaki and Kohgi ,Masahumi and Higemoto ,Wataru and E. MacLaughlin ,Douglas and Sugawara ,Hitoshi and Sato ,Hideyuki},
title = {The Unconventional Superconductivity of Skutterudite PrOs4Sb12: Time-Reversal Symmetry Breaking and Adjacent Field-Induced Quadrupole Ordering},
journal = {Journal of the Physical Society of Japan},
volume = {76},
number = {5},
pages = {051006},
year = {2007},
doi = {10.1143/JPSJ.76.051006},

URL = { 
        https://doi.org/10.1143/JPSJ.76.051006
    
},
eprint = { 
        https://doi.org/10.1143/JPSJ.76.051006
    
}
}

@article{Aoki2003,
  title = {Time-Reversal Symmetry-Breaking Superconductivity in Heavy-Fermion PrOs$_{4}$Sb$_{12}$ Detected by Muon-Spin Relaxation},
  author = {Aoki, Y. and Tsuchiya, A. and Kanayama, T. and Saha, S. R. and Sugawara, H. and Sato, H. and Higemoto, W. and Koda, A. and Ohishi, K. and Nishiyama, K. and Kadono, R.},
  journal = {Phys. Rev. Lett.},
  volume = {91},
  issue = {6},
  pages = {067003},
  numpages = {4},
  year = {2003},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.91.067003},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.91.067003}
}

@article{Yarzhemsky2009,
author="Yarzhemsky, V. G.
and Nefedov, V. I.",
title="Time-Reversal symmetry violation and the structure of the superconducting order parameter of PrOs4Sb12                  ",
journal="Physics of the Solid State",
year="2009",
month="Mar",
day="11",
volume="51",
number="3",
pages="448",
doi="10.1134/S1063783409030020",
url="https://doi.org/10.1134/S1063783409030020"
}

@article{Maisuradze2010,
  title = {Evidence for time-reversal symmetry breaking in superconducting ${\text{PrPt}}_{4}{\text{Ge}}_{12}$},
  author = {Maisuradze, A. and Schnelle, W. and Khasanov, R. and Gumeniuk, R. and Nicklas, M. and Rosner, H. and Leithe-Jasper, A. and Grin, Yu. and Amato, A. and Thalmeier, P.},
  journal = {Phys. Rev. B},
  volume = {82},
  issue = {2},
  pages = {024524},
  numpages = {5},
  year = {2010},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.82.024524},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.82.024524}
}

@article{Hillier2012,
  title = {Nonunitary Triplet Pairing in the Centrosymmetric Superconductor ${\mathrm{LaNiGa}}_{2}$},
  author = {Hillier, A. D. and Quintanilla, J. and Mazidian, B. and Annett, J. F. and Cywinski, R.},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  issue = {9},
  pages = {097001},
  numpages = {5},
  year = {2012},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.097001},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.097001}
}

@article{Hillier2012,
  title = {Evidence for Time-Reversal Symmetry Breaking in the Noncentrosymmetric Superconductor ${\mathrm{LaNiC}}_{2}$},
  author = {Hillier, A. D. and Quintanilla, J. and Cywinski, R.},
  journal = {Phys. Rev. Lett.},
  volume = {102},
  issue = {11},
  pages = {117007},
  numpages = {4},
  year = {2009},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.102.117007},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.102.117007}
}


@article{Bhattacharyya2015,
	Author = {Bhattacharyya, Amitava and Adroja, Devashibhai and Kase, Naoki and Hillier, Adrian and Akimitsu, Jun and Strydom, Andre},
	Date = {2015/08/19/online},
	Date-Added = {2018-09-05 17:25:47 +0000},
	Date-Modified = {2018-09-05 17:25:47 +0000},
	Day = {19},
	Journal = {Scientific Reports},
	L3 = {10.1038/srep12926; },
	M3 = {Article},
	Month = {08},
	Pages = {12926 EP},
	Title = {Unconventional superconductivity in Y5Rh6Sn18 probed by muon spin relaxation},
	Ty = {JOUR},
	Url = {http://dx.doi.org/10.1038/srep12926},
	Volume = {5},
	Year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/srep12926}
}

@Book{deGennes1999,
  title={Superconductivity of Metals and Alloys},
  author={Pierre-Gilles de Gennes},
  isbn={9780738201016},
  lccn={99060033},
  series={Advanced book classics},
  url={https://books.google.ca/books?id=xacsAAAAYAAJ},
  year={1999},
  publisher={Advanced Book Program, Perseus Books}
}

@Book{Bauer2012,
  title={Noncentrosymmetric Superconductors: Introduction and
Overview},
  author={E Bauer and M. Sigrist},
  year={2012},
  publisher={Springer, Berlin}
}

@Book{Tinkham1975,
author = { Tinkham, Michael. },
title = { Introduction to superconductivity},
isbn = { 0070648778 },
publisher = { McGraw-Hill New York },
year = { 1975 },
type = { Book },
subjects = { Superconductivity. },
catalogue-url = { https://nla.gov.au/nla.cat-vn1834745 }
}

@article{Bhattacharyya,
  title = {Broken time-reversal symmetry probed by muon spin relaxation in the caged type superconductor ${\mathrm{Lu}}_{5}{\mathrm{Rh}}_{6}{\mathrm{Sn}}_{18}$},
  author = {Bhattacharyya, A. and Adroja, D. T. and Quintanilla, J. and Hillier, A. D. and Kase, N. and Strydom, A. M. and Akimitsu, J.},
  journal = {Phys. Rev. B},
  volume = {91},
  issue = {6},
  pages = {060503},
  numpages = {5},
  year = {2015},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.91.060503},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.91.060503}
}

@article{Amon2018,
  title = {Noncentrosymmetric superconductor BeAu},
  author = {Amon, A. and Svanidze, E. and Cardoso-Gil, R. and Wilson, M. N. and Rosner, H. and Bobnar, M. and Schnelle, W. and Lynn, J. W. and Gumeniuk, R. and Hennig, C. and Luke, G. M. and Borrmann, H. and Leithe-Jasper, A. and Grin, Yu.},
  journal = {Phys. Rev. B},
  volume = {97},
  issue = {1},
  pages = {014501},
  numpages = {11},
  year = {2018},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.97.014501},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.97.014501}
}

@article{Wilson2017,
author = {Wilson, Murray and Hallas, Alannah and Cai, Yi-peng and Guo, S and Gong, Z and Sankar, Raman and Chou, F and J. Uemura, Y and Luke, Graeme},
year = {2017},
month = {03},
pages = {},
title = {\mu$SR study of noncentrosymmetric superconductor PbTaSe$_2},
volume = {95},
booktitle = {Physical Review B}
}

@article{Egorov2001,
  title = {Superconducting intermediate state of white tin studied by muon-spin-rotation spectroscopy},
  author = {Egorov, V. S. and Solt, G. and Baines, C. and Herlach, D. and Zimmermann, U.},
  journal = {Phys. Rev. B},
  volume = {64},
  issue = {2},
  pages = {024524},
  numpages = {5},
  year = {2001},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.64.024524},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.64.024524}
}

@incollection{Landau1948,
title = "49 - ON THE THEORY OF THE INTERMEDIATE STATE OF SUPERCONDUCTORS",
editor = "D. TER HAAR",
booktitle = "Collected Papers of L.D. Landau",
publisher = "Pergamon",
pages = "365 - 379",
year = "1965",
isbn = "978-0-08-010586-4",
doi = "https://doi.org/10.1016/B978-0-08-010586-4.50054-7",
url = "http://www.sciencedirect.com/science/article/pii/B9780080105864500547"
}

@article{Beleggia2006,
author = { M.   Beleggia  and  M.   De Graef  and  Y.   Millev },
title = {Demagnetization factors of the general ellipsoid: An alternative to the Maxwell approach},
journal = {Philosophical Magazine},
volume = {86},
number = {16},
pages = {2451-2466},
year  = {2006},
publisher = {Taylor & Francis},
doi = {10.1080/14786430600617161},

URL = { 
        https://www.tandfonline.com/doi/abs/10.1080/14786430600617161
    
},
eprint = { 
        https://www.tandfonline.com/doi/pdf/10.1080/14786430600617161
    
}

}

@article{Osborn1945,
  title = {Demagnetizing Factors of the General Ellipsoid},
  author = {Osborn, J. A.},
  journal = {Phys. Rev.},
  volume = {67},
  issue = {11-12},
  pages = {351--357},
  numpages = {0},
  year = {1945},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.67.351},
  url = {https://link.aps.org/doi/10.1103/PhysRev.67.351}
}

@article{DeGennes1964,
  title = {Boundary Effects in Superconductors},
  author = {DE GENNES, P. G.},
  journal = {Rev. Mod. Phys.},
  volume = {36},
  issue = {1},
  pages = {225--237},
  numpages = {0},
  year = {1964},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.36.225},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.36.225}
}

@article{Khan2016,
  title = {Complex superconductivity in the noncentrosymmetric compound ${\mathrm{Re}}_{6}\mathrm{Zr}$},
  author = {Khan, Mojammel A. and Karki, A. B. and Samanta, T. and Browne, D. and Stadler, S. and Vekhter, I. and Pandey, Abhishek and Adams, P. W. and Young, D. P. and Teknowijoyo, S. and Cho, K. and Prozorov, R. and Graf, D. E.},
  journal = {Phys. Rev. B},
  volume = {94},
  issue = {14},
  pages = {144515},
  numpages = {10},
  year = {2016},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.94.144515},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.94.144515}
}

@article{Biswas2013,
  title = {Evidence for superconductivity with broken time-reversal symmetry in locally noncentrosymmetric SrPtAs},
  author = {Biswas, P. K. and Luetkens, H. and Neupert, T. and St\"urzer, T. and Baines, C. and Pascua, G. and Schnyder, A. P. and Fischer, M. H. and Goryo, J. and Lees, M. R. and Maeter, H. and Br\"uckner, F. and Klauss, H.-H. and Nicklas, M. and Baker, P. J. and Hillier, A. D. and Sigrist, M. and Amato, A. and Johrendt, D.},
  journal = {Phys. Rev. B},
  volume = {87},
  issue = {18},
  pages = {180503},
  numpages = {5},
  year = {2013},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.87.180503},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.87.180503}
}

@article{Singh2016,
  title = {Superconducting properties of the noncentrosymmetric superconductor ${\mathrm{Re}}_{6}\mathrm{Hf}$},
  author = {Singh, D. and Hillier, A. D. and Thamizhavel, A. and Singh, R. P.},
  journal = {Phys. Rev. B},
  volume = {94},
  issue = {5},
  pages = {054515},
  numpages = {9},
  year = {2016},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.94.054515},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.94.054515}
}

@article{Singh2018,
  title = {Time-reversal symmetry breaking in the noncentrosymmetric superconductor ${\mathrm{Re}}_{6}\mathrm{Ti}$},
  author = {Singh, D. and K. P., Sajilesh and Barker, J. A. T. and Paul, D. McK. and Hillier, A. D. and Singh, R. P.},
  journal = {Phys. Rev. B},
  volume = {97},
  issue = {10},
  pages = {100505},
  numpages = {6},
  year = {2018},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.97.100505},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.97.100505}
}

@article{Livingston1963_1,
  title = {Magnetic Properties of Superconducting Lead-Base Alloys},
  author = {Livingston, J. D.},
  journal = {Phys. Rev.},
  volume = {129},
  issue = {5},
  pages = {1943--1949},
  numpages = {0},
  year = {1963},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.129.1943},
  url = {https://link.aps.org/doi/10.1103/PhysRev.129.1943}
}


@article{Livingston1963_2,
author = {Livingston,J. D. },
title = {Precipitation and Superconductivity in Lead‐Tin and Lead‐Cadmium Alloys},
journal = {Journal of Applied Physics},
volume = {34},
number = {10},
pages = {3028-3036},
year = {1963},
doi = {10.1063/1.1729115},

URL = { 
        https://doi.org/10.1063/1.1729115
    
},
eprint = { 
        https://doi.org/10.1063/1.1729115
    
}

}

@Book{Landau1983,
author = { Landau and Lifshitz },
title = {Electrodynamics of Continuous Media},
isbn = { 9780080570600 },
publisher = {  Butterworth-Heinemann },
pages = { 460},
year = { 1983 },
type = { Book },
catalogue-url = { https://nla.gov.au/nla.cat-vn1834745 }
}

@article {Andrew1948,
	title = {The intermediate state of superconductors III. Theory of behaviour of superconducting cylinders in transverse magnetic fields},
	volume = {194},
	number = {1036},
	pages = {98--112},
	year = {1948},
	doi = {10.1098/rspa.1948.0068},
	publisher = {The Royal Society},
	issn = {0080-4630},
	URL = {http://rspa.royalsocietypublishing.org/content/194/1036/98},
	eprint = {http://rspa.royalsocietypublishing.org/content/194/1036/98.full.pdf},
	journal = {Proceedings of the Royal Society of London A: Mathematical, Physical and Engineering Sciences}
}

@article{Fortini1972,
  title = {Thermodynamics of the Domain Structure and Determination of the Transition Fields in Type-1 Superconductors},
  author = {Fortini, Andr\'e and Paumier, Eric},
  journal = {Phys. Rev. B},
  volume = {5},
  issue = {5},
  pages = {1850--1858},
  numpages = {0},
  year = {1972},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.5.1850},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.5.1850}
}

@Book{Huebener1979,
author = { Huebener, Rudolf Peter},
title = { Magnetic flux structures in superconductors},
isbn = { 0387092137 },
publisher = { Springer-Verlag Berlin ; New York },
pages = { xi, 259 p. : },
year = { 1979 },
type = { Book },
language = { English },
subjects = { Superconductors.; Magnetic flux. },
life-dates = { 1979 -  },
catalogue-url = { https://nla.gov.au/nla.cat-vn585361 }
}

@article{Jennings1959,
  title = {Effects of Pressure on the Superconducting Transition Temperatures of Sn, In, Ta, Tl, and Hg},
  author = {Jennings, L. D. and Swenson, C. A.},
  journal = {Phys. Rev.},
  volume = {112},
  issue = {1},
  pages = {31--43},
  numpages = {0},
  year = {1958},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.112.31},
  url = {https://link.aps.org/doi/10.1103/PhysRev.112.31}
}

@article{Salis2018,
	doi = {10.1088/1361-648x/aaed31},
	url = {https://doi.org/10.1088%2F1361-648x%2Faaed31},
	year = 2018,
	month = {nov},
	publisher = {{IOP} Publishing},
	volume = {30},
	number = {50},
	pages = {505602},
	author = {M V Salis and P Rodi{\`{e}}re and H Leng and Y K Huang and A de Visser},
	title = {Penetration depth study of the type-I superconductor {PdTe}2},
	journal = {Journal of Physics: Condensed Matter},

}

@article{Bekaert2016,
  title = {Anisotropic type-I superconductivity and anomalous superfluid density in ${\mathrm{OsB}}_{2}$},
  author = {Bekaert, J. and Vercauteren, S. and Aperis, A. and Komendov\'a, L. and Prozorov, R. and Partoens, B. and Milo\ifmmode \check{s}\else \v{s}\fi{}evi\ifmmode \acute{c}\else \'{c}\fi{}, M. V.},
  journal = {Phys. Rev. B},
  volume = {94},
  issue = {14},
  pages = {144506},
  numpages = {9},
  year = {2016},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.94.144506},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.94.144506}
}

@article{Yamada2018,
author = {Yamada ,Akira and Higashinaka ,Ryuji and Matsuda ,Tatsuma D. and Aoki ,Yuji},
title = {Superconductivity in Cage Compounds LaTr2Al20 with Tr = Ti, V, Nb, and Ta},
journal = {Journal of the Physical Society of Japan},
volume = {87},
number = {3},
pages = {033707},
year = {2018},
doi = {10.7566/JPSJ.87.033707},

URL = { 
        https://doi.org/10.7566/JPSJ.87.033707
    
},
eprint = { 
        https://doi.org/10.7566/JPSJ.87.033707
    
}

}

@article{Svanidze2012,
  title = {Type-I superconductivity in ScGa${}_{3}$ and LuGa${}_{3}$ single crystals},
  author = {Svanidze, E. and Morosan, E.},
  journal = {Phys. Rev. B},
  volume = {85},
  issue = {17},
  pages = {174514},
  numpages = {5},
  year = {2012},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.85.174514},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.85.174514}
}

@article{Gottlieb1992,
  title = {Superconductivity in ${\mathrm{TaSi}}_{2}$ single crystals},
  author = {Gottlieb, U. and Lasjaunias, J. C. and Tholence, J. L. and Laborde, O. and Thomas, O. and Madar, R.},
  journal = {Phys. Rev. B},
  volume = {45},
  issue = {9},
  pages = {4803--4806},
  numpages = {0},
  year = {1992},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.45.4803},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.45.4803}
}

@article{Kriener2008,
author = {Markus Kriener and Takahiro Muranaka and Junya Kato and Zhi-An Ren and Jun Akimitsu and Yoshiteru Maeno},
title = {Superconductivity in heavily boron-doped silicon carbide},
journal = {Science and Technology of Advanced Materials},
volume = {9},
number = {4},
pages = {044205},
year  = {2008},
publisher = {Taylor & Francis},
doi = {10.1088/1468-6996/9/4/044205},

URL = { 
        https://doi.org/10.1088/1468-6996/9/4/044205
    
},
eprint = { 
        https://doi.org/10.1088/1468-6996/9/4/044205
    
}

}

@article{Smidman2014,
  title = {Investigations of the superconducting states of noncentrosymmetric LaPdSi${}_{3}$ and LaPtSi${}_{3}$},
  author = {Smidman, M. and Hillier, A. D. and Adroja, D. T. and Lees, M. R. and Anand, V. K. and Singh, R. P. and Smith, R. I. and Paul, D. M. and Balakrishnan, G.},
  journal = {Phys. Rev. B},
  volume = {89},
  issue = {9},
  pages = {094509},
  numpages = {10},
  year = {2014},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.89.094509},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.89.094509}
}

@article{Wakui2009,
author = {Wakui ,Kouhei and Akutagawa ,Satoshi and Kase ,Naoki and Kawashima ,Kenji and Muranaka ,Takahiro and Iwahori ,Yasufumi and Abe ,Jiro and Akimitsu ,Jun},
title = {Thermodynamic Properties of the Non-centrosymmetric Type-I Superconductor Rh2Ga9 and Ir2Ga9},
journal = {Journal of the Physical Society of Japan},
volume = {78},
number = {3},
pages = {034710},
year = {2009},
doi = {10.1143/JPSJ.78.034710},

URL = { 
        https://doi.org/10.1143/JPSJ.78.034710
    
},
eprint = { 
        https://doi.org/10.1143/JPSJ.78.034710
    
}
}

@article{Kimara2005,
  title = {Pressure-Induced Superconductivity in Noncentrosymmetric Heavy-Fermion ${\mathrm{CeRhSi}}_{3}$},
  author = {Kimura, N. and Ito, K. and Saitoh, K. and Umeda, Y. and Aoki, H. and Terashima, T.},
  journal = {Phys. Rev. Lett.},
  volume = {95},
  issue = {24},
  pages = {247004},
  numpages = {4},
  year = {2005},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.95.247004},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.95.247004}
}

@article{Honda2010,
  title = {Pressure-induced superconductivity and large upper critical field in the noncentrosymmetric antiferromagnet ${\text{CeIrGe}}_{3}$},
  author = {Honda, F. and Bonalde, I. and Shimizu, K. and Yoshiuchi, S. and Hirose, Y. and Nakamura, T. and Settai, R. and \ifmmode \bar{O}\else \={O}\fi{}nuki, Y.},
  journal = {Phys. Rev. B},
  volume = {81},
  issue = {14},
  pages = {140507},
  numpages = {4},
  year = {2010},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.81.140507},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.81.140507}
}


@article{Settai2007,
title = "Pressure-induced superconductivity in CeCoGe3 without inversion symmetry",
journal = "Journal of Magnetism and Magnetic Materials",
volume = "310",
number = "2, Part 1",
pages = "844 - 846",
year = "2007",
note = "Proceedings of the 17th International Conference on Magnetism",
issn = "0304-8853",
doi = "https://doi.org/10.1016/j.jmmm.2006.10.717",
url = "http://www.sciencedirect.com/science/article/pii/S0304885306019561",
author = "R. Settai and I. Sugitani and Y. Okuda and A. Thamizhavel and M. Nakashima and Y. Ōnuki and H. Harima",
}

@article{Yasuda2004,
author = {Yasuda ,Takashi and Shishido ,Hiroaki and Ueda ,Taiki and Hashimoto ,Shin and Settai ,Rikio and Takeuchi ,Tetsuya and D Matsuda ,Tatsuma and Haga ,Yoshinori and Ōnuki ,Yoshichika},
title = {Superconducting Property in CePt3Si under Pressure},
journal = {Journal of the Physical Society of Japan},
volume = {73},
number = {7},
pages = {1657-1660},
year = {2004},
doi = {10.1143/JPSJ.73.1657},

URL = { 
        https://doi.org/10.1143/JPSJ.73.1657

    
}
}

@article{Mizuguchi2008,
author = {Mizuguchi,Yoshikazu  and Tomioka,Fumiaki  and Tsuda,Shunsuke  and Yamaguchi,Takahide  and Takano,Yoshihiko },
title = {Superconductivity at 27K in tetragonal FeSe under high pressure},
journal = {Applied Physics Letters},
volume = {93},
number = {15},
pages = {152505},
year = {2008},
doi = {10.1063/1.3000616},

URL = { 
        https://doi.org/10.1063/1.3000616
    
},
eprint = { 
        https://doi.org/10.1063/1.3000616
    
}

}

@article{Singh2019,
Author = {D. Singh and A. D. Hillier and R. P. Singh},
Title = {Type-I superconductivity in noncentrosymmetric superconductor AuBe},
Year = {2019},
Eprint = {arXiv:1901.06492},
}
